Scalable Panel Fusion Using Distributed Min Cost Flow

Modern audience measurement requires combining observations from disparate panel datasets. Connecting and relating such panel datasets is a process termed panel fusion. This paper formalizes the panel fusion problem and presents a novel approach to solve it. We cast the panel fusion as a network flow problem, allowing the application of a rich body of research. In the context of digital audience measurement, where panel sizes can grow into the tens of millions, we propose an efficient algorithm to partition the network into sub-problems. While the algorithm solves a relaxed version of the original problem, we provide conditions under which it guarantees optimality. We demonstrate our approach by fusing two real-world panel datasets in a distributed computing environment.

==> methodology.tex <==
    Let C is the census panel set with n1 panelists and T is the traditional panel set with n2 panelists. \\
    For every i $\in$ C with projection weight $Cw_{i}$ and j $\in$ T with projection weight $Tw_{j}$.\par
    Both sets have same demo IDs \{d1, d2, ... $d_{k}$\} and online behavior is categorized in internet categories \{cat1, cat2, cat3, ..., $cat_{l}$\} \par
Both panel sets represents same universe. Therefore, \par 
\begin{equation}
\sum_{i=1}^{n1} Cw_{i} = \sum_{j=1}^{n2} Tw_{j}
\end{equation}

\par
Matching of C\`\ $\in$ C with T\`\ $\in$ T is considered good only with below constraints in order of strictness:\par
\begin{enumerate}[label=(\Roman*)]
  \item Weights of assigned panelists need to be perfectly aligned. Assignment of $C`_{i}$ to $T`_{j}$ can be m:n.\\
Therefore, 
$$ \sum(C`_{weights})= \sum(T`_{weights}) $$

  \item Demographic profiles of C` and T` should be as similar as possible.
  
  \item Online behavior of C` and T` also should be as similar as possible.
\end{enumerate}

    Above matching problem quickly adds complexity to generic assignment problem due to m:n matches. In general, assignment constraints as defined in [2] implies 1:1 assignment of agents(jobs) with tasks(machine) which contains a finite solution set of n! combinations. Our problem needs to generate m:n assignment because of inequality of number of panelists in two sets. (n1 $\neq$ n2).\par
m:n assignment generate infinite set of matches compared to n! which makes it computationally expensive to find solution with optimal match combinations.

\subsection{Panel matching as transportation problem}
                
Generic assignment problem is a special case of transportation problem which can be solved by minimum-cost circulation algorithms. In order to discuss this problem we define terminologies similar to [4]. \par
Let G = (V, E) where V is node set and E is edge set. Each arc(i, j) $\in$ E has an associated $\mathit{cost}$ $c_{i,j}$ per unit flow on that arc. Each arc (i, j) $\in$ E also has a $\mathit{capacity}$ $u_{i,j}$ denoting maximum amount that can flow on the arc and $\mathit{lower \ bound}$ $l_{i,j}$ denoting the minimum amount that must flow on the arc. Let an integer value b(i) represents supply/demand for each node i $\in$ V. if b(i) > 0, then node i is $\mathit{supply \ node}$; if b(i) < 0, then node i is $\mathit{demand \ node}$; and if b(i) = 0 then node i is a $\mathit{transshipment \ node}$. \par
    Minimum cost flow problem is to determine a path with least cost through  flow network satisfying the demand at demand nodes from available supplies at supply nodes. Let the flow on an arc(i, j) $\in$ E by $x_{i,j} $.  Minimum cost flow problem is an optimization model as follows: \par
 
    \begin{subequations}
    \begin{equation}
    Minimize \sum_{(i,j) \in E} c_{i,j} \ x_{i, j}
    \end{equation} \\
    \begin{equation}
    \sum_{[j : (i,j) \in E]} x_{i,j} - \sum_{[j : (i,j) \in E]} x_{j,i} = b(i), for \ all \ i \in V,
    \end{equation} \\
    \begin{equation}
    l_{i,j} \leq x_{i,j} \leq u_{i,j} \ for \ all \ (i, j) \in E
    \end{equation}   
     \end{subequations}
\\    
Constraint (3b) states that net flow out of each node must equal to supply/demand of the node. For transshipment node it will be 0. [4] refers it as $\mathit{mass \ balance \ constraint}$.\\
Constraint (3c) represents $\mathit{flow \ bound \ constraint}$ which states that flow in all arcs is bounded by that arc's lower and upper capacities.
    
\subsection{Transformation}
Following terminology defined above, G(V, E) be a fully dense bipartite graph, where V can be partitioned into two disjoint subsets C (census panelists set), T (traditional panelists set), where, \\
\indent |C| = n1 \\
\indent |T| = n2 \\
\indent |E| = n1 * n2 \\
\indent Node i $\in$ C with $\mathit{supply \ b(i)}$ = $Cw_{i}$ \\ 
\indent Node j $\in$ T with $\mathit{demand \ b(j)}$ = -$Tw_{j}$ \\
\indent Arc $(i,j)_{[i \in C,  j \in T]}$ has, \\
\indent \indent  $\mathit{capacity \ upper \ bound} \ u(i, j) $ = $\infty$ \\
\indent \indent $\mathit{capacity \ lower \ bound} \ l(i, j) $ = 0. \\
\indent \indent $\mathit{cost \ c(i,j) = d(i, j)}$ where d is a distance between i and j \\

$\mathit{b(i)}$ is set to projection weights of given panelist to meet criteria \Romannum{1}. This will make sure that weights are always aligned for matched panelists. $\mathit{u(i, j)}$ is considered $\infty$ for simplicity of explanation but can be changed to influence flow where needed. As many practical applications, $\mathit{l(i, j)}$ is assumed to be 0 to allow discarding certain edges in optimal solution if helpful.
Criteria \Romannum{2} and \Romannum{3} can be imposed with $\mathit{cost \ function \ c(i, j)}$. Demographic and online behavior features can be normalized and represented as a distance between two panelists. We used Euclidean distance function for the same. (SHOULD WE EXPLAIN THIS MORE?) \\

Illustration diagram - 
[Add a census table with demos and categories and traditional panel with same. Add a table with normalized features and Euclidean distance between them.
Then draw dense bipartite graph with all information.

 [2] = Linear assignment problems and extensions, Rainer R. Burkard, Eranda Cela.    
 [3] = Finding minimum-cost flows by double scaling - Ravindra K. ahuja
 [4] = Applications of network optimization Ravindra K. Ahuja, Thomas L. Magnati

